Jet Quenching in Relativistic Heavy Ion Collisions at the LHC

Jet production in relativistic heavy ion collisions is studied using Pb+Pb collisions at a center of mass energy of 2.76 TeV per nucleon. The measurements reported here utilize data collected with the ATLAS detector at the LHC from the 2010 Pb ion run corresponding to a total integrated luminosity of 7 inverse microbarns. The results are obtained using fully reconstructed jets using the anti-kt algorithm with a per-event background subtraction procedure. A centrality-dependent modification of the dijet asymmetry distribution is observed, which indicates a higher rate of asymmetric dijet pairs in central collisions relative to peripheral and pp collisions. Simultaneously the dijet angular correlations show almost no centrality dependence. These results provide the first direct observation of jet quenching. Measurements of the single inclusive jet spectrum, measured with jet radius parameters R = 0.2,0.3,0.4 and 0.5, are also presented. The spectra are unfolded to correct for the finite energy resolution introduced by both detector effects and underlying event fluctuations. Single jet production, through the central-to-peripheral ratio RCP, is found to be suppressed in central collisions by approximately a factor of two, nearly independent of the jet pT. The RCP is found to have a small but significant increase with increasing R, which may relate directly to aspects of radiative energy loss.

==> Makefile <==
CLEANEXTS       = aux log out bak blg bbl toc lof lot


all:    clean
	pdflatex main;\
	bibtex main;\
	pdflatex main;\
	pdflatex main

fast:
	pdflatex main

clean:
	for file in $(CLEANEXTS); do rm -f *.$$file; \
	done
        
pdf:
	@if [ -f main.ps ]; then rm main.ps; fi
	@if [ -f main.pdf ]; then rm main.pdf; fi
	@make
	@dvips -t letter main.dvi -o main.ps
	@ps2pdf main.ps
	@rm main.ps

.PHONY: all fast clean pdf
